Rainblock: Faster Transaction Processing in Public Blockchains

Public blockchains like Ethereum use Merkle trees to verify transactions received from untrusted servers before applying them to the blockchain. We empirically show that the low throughput of such blockchains is due to the I/O bottleneck associated with using Merkle trees for processing transactions. We present RAINBLOCK, a new architecture for public blockchains that increases throughput without affecting security. RAINBLOCK achieves this by tackling the I/O bottleneck on two fronts: first, decoupling transaction processing from I/O, and removing I/O from the critical path; second, reducing I/O amplification by customizing storage for blockchains. RAINBLOCK uses a novel variant of the Merkle tree, the Distributed Sharded Merkle tree (DSM-TREE) to store system state. We evaluate RAINBLOCK using workloads based on public Ethereum traces (including smart contracts) and show that RAINBLOCK processes 20K transactions per second in a geo-distributed setting with four regions spread across three continents.

==> fig-cryptokitties.tex <==
\begin{figure}
\hrule
\begin{algorithmic}[1]
  \footnotesize
  \vspace{5pt}
\Function{giveBirth}{matronId}
\State Kitty $\textit{matron} \gets kitties[matronId]$
\State $assert(matron.isValid)$
\State $assert(matron.isReadyToGiveBirth)$\\
\State Kitty $\textit{sire} \gets kitties[matron.sireId]$
\State $\textit{childGenes} \gets mixGenes(matron.genes, sire.genes)$
\State $\textit{newKitty} \gets createKitty(matron, sire, childGenes)$
\State $\textit{pregnantKitties}--$
\State $sender.send(birthFee)$
\State \textbf{return} $newKitty$
\EndFunction
\end{algorithmic}
\vspace{5pt}
\hrule
    \caption{\emph{Fixed-address contract example.} Psuedocode of the CryptoKitties \texttt{giveBirth} function, which indicates that storage reads (accesses to the \texttt{kitties} array) only depend on function arguments.}
    \label{fig:cryptokitties}
\end{figure}


==> fig-revision.tex <==
\begin{figure}
  \includegraphics[width=\columnwidth]{figures/revision-new1.pdf}
  \mycaption{Witness Revision} {Transaction tx1 has been applied to
    \dsm cache, with the changed nodes shaded.  When tx2 arrives, node
    C is stale in its node bag. The miner automatically revises this
    node during traversal, adopting node C' instead to reach hash node
    G, which it retrieves from the node bag to fetch the leaf node for
    account $657$.}
    \label{fig:revision}
    %\vspace{-0.2in}
\end{figure}


==> tbl-dsm-optimizations.tex <==
\begin{table}[]
  \centering
  \begin{tabular}{@{}l|l@{}}
  \toprule
    \dsm design &
    Summary and Benefits
    \\ \midrule

    \begin{tabular}[c]{@{}l@{}}
      In-memory\\
      representation
    \end{tabular} &
    \begin{tabular}[c]{@{}l@{}}
      (1) Avoids redundant \io amplification\\
      (2) Allows lazy hash resolution\\
      (3) Makes Merkle tree traversals faster
    \end{tabular}
    \\ \midrule

    \begin{tabular}[c]{@{}l@{}}
      Lazy hash\\
      resolution
    \end{tabular} &
    \begin{tabular}[c]{@{}l@{}}
      Defers hash computations till needed\\
      (1) Reduces number of hash computations\\
      (2) Reduces expensive node serializations
    \end{tabular}
    \\ \midrule

    \begin{tabular}[c]{@{}l@{}}
      Node bags
    \end{tabular} &
    \begin{tabular}[c]{@{}l@{}}
      Deduplicates Merkle nodes across witnesses\\
      (1) Helps batches multiple witnesses\\
      (2) Reduces witness sizes and network traffic
    \end{tabular}
    \\ \midrule

    \begin{tabular}[c]{@{}l@{}}
      Witness Revision
    \end{tabular} &
    \begin{tabular}[c]{@{}l@{}}
      Updates a slightly stale but correct witness\\
      (1) Allows executing some transactions\\
      which would otherwise get aborted
    \end{tabular}
    \\ \midrule

    \begin{tabular}[c]{@{}l@{}}
      Witness\\
      Compaction
    \end{tabular} &
    \begin{tabular}[c]{@{}l@{}}
      Bottom layer sends partial witnesses as the\\
      top layer can verify them\\
      (1) Reduces witness sizes and network traffic
    \end{tabular}
    \\ \bottomrule
  \end{tabular}
  \mycaption{\dsms design and their benefits}{This table summarizes the
  core design optimizations in \dsm.}
  \label{tab:dsm-optimizations}
  \vspace{-15pt}
  \end{table}

==> tbl-principles.tex <==
\begin{table}[]
  \centering
  \begin{tabular}{@{}l|l@{}}
  \toprule
  \sysname core principle &
    Benefits and goals
    \\ \midrule
  \begin{tabular}[c]{@{}l@{}}Decoupling authentication\\ of state from miners\end{tabular} &
    \begin{tabular}[c]{@{}l@{}}Helps tackle \io bottlenecks\\ without assuming hardware\\ limitations on miners\end{tabular}
    \\ \midrule
    \begin{tabular}[c]{@{}l@{}}Prefetching data out of\\ the critical path\end{tabular} &
    \begin{tabular}[c]{@{}l@{}}Helps miners avoid performing\\ \io in the critical path of\\ processing transactions\end{tabular}
    \\ \midrule
    \begin{tabular}[c]{@{}l@{}}Customizing storage\\ for public blockchains\end{tabular} &
    \begin{tabular}[c]{@{}l@{}}Eliminates \io amplification from\\ using key-value stores like\\ RocksDB to store Merkle trees\end{tabular}
    \\ \bottomrule
  \end{tabular}
  \mycaption{\sysname design principles}{This table highlights the three core design principles of \sysname architecture.}
  \label{tab:principles}
  \vspace{-20pt}
\end{table}
